GSum: A General Framework for Guided Neural Abstractive Summarization

Neural abstractive summarization models are flexible and can produce coherent summaries, but they are sometimes unfaithful and can be difficult to control. While previous studies attempt to provide different types of guidance to control the output and increase faithfulness, it is not clear how these strategies compare and contrast to each other. In this paper, we propose a general and extensible guided summarization framework (GSum) that can effectively take different kinds of external guidance as input, and we perform experiments across several different varieties. Experiments demonstrate that this model is effective, achieving state-of-the-art performance according to ROUGE on 4 popular summarization datasets when using highlighted sentences as guidance. In addition, we show that our guided model can generate more faithful summaries and demonstrate how different types of guidance generate qualitatively different summaries, lending a degree of controllability to the learned models.

==> background.tex <==
\section{Background}
\subsection{Neural Summarization}
In this part, we will introduce both the extractive and abstractive neural summarization models.

\paragraph{Extractive Summarization.} Extractive summarization models generate a summary by selecting and concatenating the most important sentences in a document. To this end, the summarization task is typically formalized as a sentence-level classification problem for neural approaches. Specifically, each sentence will be assigned with a probability of whether it should be included in the output and $k$ sentences with the highest probabilities will be selected, where $k$ is a hyper-parameter and is dataset-dependent. 

Because most summarization corpora only contain human-generated summaries, heuristics are often used to obtain an oracle summary for each summary. For example,~\citet{nallapati2017summarunner} and~\citet{liu2019text} employ a greedy approach that incrementally add one sentence to the summary, and the sentence that can increase the ROUGE score with the entire human-written summary the most will be selected at each step. 

It should be noted that there are also neural approaches that do not adopt this paradigm. For example,~\citet{Zhang2018NeuralLE} directly maximize the likelihood of human summaries given selected sentences and~\citet{zhong2020extractive} formulate the extractive summarization task as a semantic text matching problem and achieve state-of-the-art performance on almost all popular benchmarks.

\paragraph{Abstractive Summarization.} Sequence-to-sequence framework~\citep{seq2seq1,seq2seq2} with the attention mechanism~\citep{Bahdanau2015NeuralMT} is usually adopted in current neural abstractive summarization approaches, where an encoder generates a context vector for each source sentence and a decoder then outputs a summary, one target word at a time. 

While being conceptually simple, neural abstractive summarization models can suffer from generating unfaithful summaries. To alleviate such a problem, copy mechanism is introduced in the field of text summarization~\citep{gu2016incorporating,see2017get,gehrmann2018bottom}, which allows the model to learn to detect important words or phrases in the source side and directly copy them to the target side with certain probabilities.

Current state-of-the-art abstractive summarization model mainly utilize pre-trained language models. For example,~\citet{liu2019text} use the pretrained BERT model~\citep{Devlin2019BERTPO} to initialize the encoder of summarization models and then fine-tune the model on summarization datasets. Similarly,~\citet{Lewis2019BARTDS} pretrain a language model with a denoising autoencoding objective and fine-tune it on summarization datasets.






% \pfliu{Or, we can also organize our related work section in this way and put it here.}


% \begin{table}[htbp]
%   \centering
%   \caption{\textit{Type} denotes different guided information. \textit{encStructure} represents how guided information is introduce.}
%     \begin{tabular}{llcc}
%     \toprule
%     \textbf{Work} & \textbf{Type} & \multicolumn{1}{l}{\textbf{encStructure}} & \multicolumn{1}{l}{\textbf{Training}} \\
%     \midrule
%     cite1 & highSent & -     & - \\
%     cite2 & keywords & -     & - \\
%     cite3 & keywords & -     & - \\
%     cite4 & softTemp & -     & - \\
%     cite5 & softTemp & -     & - \\
%     \midrule
%     ours  & all   & self-att & oracle \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%

